Low Complexity Hybrid Beamforming for mmWave Full-Duplex Integrated Access and Backhaul

We consider an integrated access and backhaul (IAB) node operating in full-duplex (FD) mode. We analyze simultaneous transmission from the New Radio gNB to the IAB node on the backhaul uplink, IAB node to a user equipment (UE) on the access downlink, and IAB transmitter to the IAB receiver on the self-interference (SI) channel. Our contributions include (1) a low complexity algorithm to jointly design the hybrid analog/digital beamformers for all three nodes to maximize the sum spectral efficiency of the access and backhaul links by canceling SI and maximizing received power; (2) derivation of all-digital beamforming and spectral efficiency upper bound for use in benchmarking; and (3) simulations to compare full vs. half duplex modes, hybrid vs. all-digital beamforming algorithms, proposed hybrid vs. conventional beamforming algorithms, and spectral efficiency upper bound. In simulations, the proposed algorithm shows significant reduction in SI power and increase in sum spectral efficiency.

==> performance.tex <==
\section{Performance Analysis}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/hardware.pdf}
    \caption{Basic abstraction of a hybrid combiner.}
    \label{system}
\end{figure}
\subsection{Energy Efficiency}
The energy efficiency, expressed in bits/s/Watt or bits/Joule, is defined as the ratio between the spectral efficiency and the total power consumption. It is expressed as
\begin{equation}
\mathcal{J}(\mathsf{sqinr}) = \frac{\mathcal{I}(\mathsf{sqinr})}{\rho_{\text{Total}}}    
\end{equation}
Where $\rho_{\text{Total}}$ is the total power consumption. For full-digital and hybrid combiners (DC and HC), the total power consumption model for each architecture is defined by
\begin{equation}
\rho^{\text{DC}}_{\text{Total}} =   N_{\text{RX}} \left(\rho_{\text{LNA}} + \rho_{\text{RF}} + 2\rho_{\text{ADC}}  \right) 
\end{equation}
\begin{equation}
\rho^{\text{HC}}_{\text{Total}} = N_{\text{RX}}\left( \rho_{\text{LNA}} + \rho_{\text{SP}} + N_{\text{RF}}\rho_{\text{PS}}  \right) +  N_{\text{RF}} \left( \rho_{\text{RF}} + \rho_{\text{C}} + 2\rho_{\text{ADC}} \right)
\end{equation}
Where $\rho_{\text{RF}}$ is the power consumption per RF chain which is defined by
\begin{equation}
\rho_{\text{RF}} = \rho_{\text{M}} + \rho_{\text{LO}} + \rho_{\text{LPF}} + \rho_{\text{B}\text{B}_{\text{amp}} }    
\end{equation}
\begin{table}[H]
\renewcommand{\arraystretch}{1}
\caption{Power Consumption of Each Device \cite{adc}.}
\label{param}
\centering
\begin{tabular}{rll}
\bfseries Device & \bfseries Notation & \bfseries Value\\
\hline
Low Noise Amplifier (LNA) \cite{adc36} & $\rho_{\text{LNA}}$ & 39 mW\\
Splitter & $\rho_{\text{SP}}$ & 19.5 mW\\
Combiner \cite{adc36} & $\rho_{\text{C}}$ & 19.5 mW\\
Phase Shifter \cite{adc37,adc38} & $\rho_{\text{PS}}$ & 2 mW\\
Mixer \cite{adc39} & $\rho_{\text{M}}$  & 16.8 mW\\
Local Oscillator \cite{adc27} & $\rho_{\text{LO}}$ & 5 mW\\
Low Pass Filter \cite{adc27} & $\rho_{\text{LPF}}$ & 14 mW\\
Baseband Amplifier \cite{adc27} & $\rho_{\text{B}\text{B}_{\text{amp}} }$ & 5 mW\\
ADC & $\rho_{\text{ADC}}$ & $cB2^b$
\end{tabular}
\end{table}

\begin{table}[H]
\renewcommand{\arraystretch}{1}
\caption{ADC Power Consumption Per Sample Per Level, $c$ \cite{adc}.}
\label{param}
\centering
\begin{tabular}{rll}
\bfseries Scenario & \bfseries Value & \bfseries Generation\\
\hline
LPADC & 5 fJ/step/Hz & Ideal future value\\
IPADC & 65 fJ/step/Hz & Intermediate Power\\
HPADC & 494 fJ/step/Hz & State of the art\\
\end{tabular}
\end{table}

\subsection{Outage Probability}
Once a transmission strategy is specified, the corresponding outage probability for rate $R$ (bits/s/Hz) is then
\begin{equation}
    P_{\textsf{out}}(\mathsf{sqinr}, R) = \mathbb{P}[\mathcal{I}(\mathsf{sqinr})<R ].
\end{equation}
With convenient powerful channel codes, the probability of error when there is no outage is very small and hence the outage probability is an accurate approximation for the actual block error probability. As justified in the literature, modern radio systems such as UMTS and LTE operate at a target error probability. Therefore, the primary performance metric is the maximum rate\footnote[2]{In this work, we define the notion of rate with outage as the average data rate that is correctly received/decoded at the receiver which is equivalent to the throughput. In other standards in the literature, the rate with outage is assimilated with the transmit data rate. The only difference is if we consider rate with outage as the throughput, we account for the probability of bursts (outage) and we multiply by the term (1-$\epsilon$), while for the transmit data rate, the term (1-$\epsilon$) is not accounted anymore.}, at each $\mathsf{sqinr}$, such that this threshold is not overtaken, i.e.,
\begin{equation}
R_\epsilon(\mathsf{sqinr}) = \max_{\zeta}\left\{ \zeta: P_{\textsf{out}}(\mathsf{sqinr}, \zeta) \leq \epsilon \right\}
\end{equation}
where $\epsilon$ is the target.
